Digital Reconstruction of Elmina Castle for Mobile Virtual Reality via Point-based Detail Transfer

Reconstructing 3D models from large, dense point clouds is critical to enable Virtual Reality (VR) as a platform for entertainment, education, and heritage preservation. Existing 3D reconstruction systems inevitably make trade-offs between three conflicting goals: the efficiency of reconstruction (e.g., time and memory requirements), the visual quality of the constructed scene, and the rendering speed on the VR device. This paper proposes a reconstruction system that simultaneously meets all three goals. The key idea is to avoid the resource-demanding process of reconstructing a high-polygon mesh altogether. Instead, we propose to directly transfer details from the original point cloud to a low polygon mesh, which significantly reduces the reconstruction time and cost, preserves the scene details, and enables real-time rendering on mobile VR devices. While our technique is general, we demonstrate it in reconstructing cultural heritage sites. We for the first time digitally reconstruct the Elmina Castle, a UNESCO world heritage site at Ghana, from billions of laser-scanned points. The reconstruction process executes on low-end desktop systems without requiring high processing power, making it accessible to the broad community. The reconstructed scenes render on Oculus Go in 60 FPS, providing a real-time VR experience with high visual quality. Our project is part of the Digital Elmina effort (http://digitalelmina.org/) between University of Rochester and University of Ghana.

==> ack.tex <==
%
% The acknowledgments section is defined using the "acks" environment
% (and NOT an unnumbered section). This ensures the proper
% identification of the section in the article metadata, and the
% consistent spelling of the heading.

\begin{acks}
We thank Prof. Yuhao Zhu for guiding and support. We also thank Prof. Michael Jarvis of the Digital History Lab of University of Rochester for providing us with the research background problem and the laser scans of the Rush Rhees Library statue and Elmina Castle in Ghana. 
\end{acks}



==> disc.tex <==
\section{Discussion}

The render result comparison shows effectiveness for applying details transfer, especially color details transfer, to a low polygon mesh with high polygon count mesh intermediate. While we are still implementing direct details transfer from point clouds, we are confident that since the high polygon count mesh will loose some details during reconstruction, direct transfer from point clouds will help retain more details than high polygon count mesh and hence produce a better result.

Note that in the result comparison, if one compares closely between the low polygon count mesh with feature transfer and the high polygon count mesh, one can spot the roughness of the lower polygon mesh. This shows that while details transfer may not make up the geometry details provided by more polygons, it can still be an effective method to provide low polygon count mesh for mobile VR/AR applications with relatively high details, especially in applications where users won't be inspecting the meshes closely. The fact that normal details transfer will reduce rendered frame quality assessed by RMSE and PSNR is contradicting to visual inspection and intuition since normal details are capable of increasing variation in light reflection patterns. We are unsure what causes this contradiction and can be a topic of further investigation.


==> pseudocode.tex <==
%https://tex.stackexchange.com/questions/64204/mutliple-inputs-with-line-breaking
\newlength\mylen
\newcommand\myinput[1]{%
  \settowidth\mylen{\KwIn{}}%
  \setlength\hangindent{\mylen}%
  \hspace*{\mylen}#1\\}

\begin{algorithm2e}[t]
\SetAlgoLined
\SetKwProg{Fn}{function}{}{}
\KwIn{Point cloud $\mathbb{P}$ represented as an octree;}
\myinput{Mesh $\mathbb{M}$ constructed from $\mathbb{P}$;}
\myinput{UV map $\mathbb{U}$ unwrapped from $\mathbb{M}$.}
\KwResult{Texture map $\mathbb{T}$; Normal map $\mathbb{N}$.}

\Fn{\funcname{Transfer}($\mathbb{P}$, $\mathbb{M}$, $\mathbb{U}$)}{
  \ForEach{Triangle $m$ in $\mathbb{M}$} {
    \tcp{Find points in $\mathbb{P}$ that are likely on $m$}
    $P \leftarrow \funcname{findPointsInPointCloud}(\mathbb{P}, m)$;\\
    \BlankLine
    \tcp{Map $P$ to the UV map $\mathbb{U}$}
    \ForEach{Point $p$ in $P$} {
      $c \leftarrow$ project $p$ to $m$ along $m$'s normal and return the barycentric coordinates of $p$ w.r.t. $m$;\\
      $q \leftarrow$ the point in $t$ whose barycentric coordinates are the same as $c$;\\
      $Q$ += $q$;\\
    }
    \BlankLine
    $t \leftarrow$ triangle in $\mathbb{U}$  corresponding to $m$;\\
    $S \leftarrow$ Triangulate($Q$, $t$.vertices);\\
    \tcp{Rasterize $t$ by triangular interpolation}
    \ForEach{Pixel $x$ in Triangle $t$}{
      $s \leftarrow$ the triangle in $S$ that bounds $x$;\\
      $\mathbb{N}[x] \leftarrow$ interpolating $x$'s normal from $s$;\\
      $\mathbb{T}[x] \leftarrow$ interpolating $x$'s color from $s$;\\
    }
    
  }
  \Return $\mathbb{T}$, $\mathbb{N}$;
}
\BlankLine
\Fn{\funcname{findPointsInPointCloud}($\mathbb{P}$, $m$)}{
  $P = \emptyset$;\\
  $N \leftarrow$ the octree node in $\mathbb{P}$ that bounds $m$;\\
  \ForEach{Point $p$ in $N$} {
    \If{$distance(p, m) \leq threshold_d$ $\&\&$ $angle(p.normal, m.normal \leq threshold_n$} {
      $P$.add($p$);
    }
  }
  \Return $P$;
}

\caption{Details transfer from a colored point cloud to a UV map, which is unwrapped from a mesh that is constructed from the point cloud.}
\label{alg:trans}
\end{algorithm2e}

